The Hidden Power of Pure 16-bit Floating-Point Neural Networks

Lowering the precision of neural networks from the prevalent 32-bit precision has long been considered harmful to performance, despite the gain in space and time. Many works propose various techniques to implement half-precision neural networks, but none study pure 16-bit settings. This paper investigates the unexpected performance gain of pure 16-bit neural networks over the 32-bit networks in classification tasks. We present extensive experimental results that favorably compare various 16-bit neural networks' performance to those of the 32-bit models. In addition, a theoretical analysis of the efficiency of 16-bit models is provided, which is coupled with empirical evidence to back it up. Finally, we discuss situations in which low-precision training is indeed detrimental.

==> temp.tex <==
\subsection{Future}
Using 16-bit floating-point precision, also known as "half precision," can significantly reduce the computational time for training and deploying convolutional neural networks maintaining the test accuracy. This is particularly useful for large-scale models and for devices with limited computational resources.

According to the results of the experiment, a more complex and powerful model can be created with 16 bits compared to the same computational time with 32-bit. However, there are still several challenges associated with using lower precision in deep learning. For example, as previously mentioned, the introduction of numerical instability can negatively impact the model's performance. Additionally, there are a limited number of optimizers' hyperparameters that support 16-bit precision, and there are also challenges associated with implementing batch normalization at lower precision.

Despite these challenges, the use of 16-bit precision is an important research in the field of deep learning, and it is expected to continue to be an important area of focus in the near future. As the field continues to progress, it is likely that more efficient and accurate 16-bit-based models will be developed, which will be beneficial for a wide range of applications.


\subsection{Optimizers (OLD)}
We found that when we used other optimizers with default settings, except Mini-Batch (SGD), 16-bit neural network caused the learning process to stop. However, by adjusting the only one hyperparameter called epsilon, we were able to successfully use 16-bit neural network with other optimizers including RMSProp and Adam. We explain the reason why optimizers can work on 16-bit Neural Network.
\begin{align*}
\theta =& \theta - \eta \nabla_{\theta} J(\theta)
\end{align*} 
Where $\theta$ is the model's parameters, $\eta$ is the learning rate, and $\nabla_{\theta} J(\theta)$ is the gradient of the loss function $J(\theta)$ with respect to the parameters.

\subsubsection{Mini-Batch Gradient Descent}
Mini-batch gradient descent is a variant of the gradient descent algorithm that divides the training datasets into small batches to compute errors (Ruder \$ Sebastian, 2016). The update rule for the parameters in mini-batch gradient descent can be written as:
\begin{align*}
\theta =& \theta - \eta \nabla_{\theta} J(\theta; x^{(i:i+n)}; y^{(i:i+n)})
\end{align*} 
This optimizer uses mini-batches of $m$ examples $(x^{(i:i+n)}, y^{(i:i+n)})$ from the training dataset ${x^{(i)},..., x^{(n)}}$ to update the model's parameters $\theta \in \mathbb{R}^{d}$ and minimize the function $J(\theta)$ by taking steps in the opposite direction of the gradient of the function with respect to the parameters (Bottou, 2010). The size of these steps is determined by the learning rate $\eta$. We think Mini-Batch Gradient Descent will work well on 16-bit as well, since the number of Hyperparameters that can cause numerical instability inside of neural network is small when minimizing $J(\theta)$.

\textbf{Assumption 3.1} \textit{We assume that input image data $x \in X\{x_1,…,x_i\}$, label $y \in Y\{y_1,…,y_i\}$, all $x \in \mathbb{R}$, $0<x<255$, all $y \in \mathbb{Z}$. Data Normalized $\bar{x}$ will be range in $0.0<\Bar{x}<1.0$. Then, if $fp16_{min}<f(x,y)=\nabla_{\theta} J(\theta; x^{(i)}; y^{(i)}) )<fp16_{max}$, and $f(x,y)$ does not cause numerical instability $I=\{NaN, Inf\}$ in updating the $\theta$, the mini-batch gradient descent works for training the 16-bit neural network.}

According to \textbf{Assumption 3.1}, there are not many hyperparameters in the Mini-Batch Gradient Descent that will cause numerical instability. the optimizer will work on 16-bit neural networks with default hyperparameter.

\subsubsection{RMSProp}
Root Mean Square Propagation is a gradient-based optimization technique used in training neural networks proposed by Geoff Hinton in Lecture 6e of his Coursera Class. Unlike 32-bit, 16-bit neural network compiled with RMSProp optimizer using default hyperparameters, weights become $NaN$, and training does not perform at all. We can avoid this numerical issue if we find the reason of numerical instability in RMSProp optimizer on 16-bit environments. The update rule of RMSProp can be written as:
\begin{align*}
w_t =& w_{t-1} - \eta \frac{g_t}{\sqrt{v_t} + \epsilon}
\end{align*}
The 16-bit floating point has a limited computational range compared to the 32-bit floating point. If it is out of range of $fp16$, numerical instability occurs in training sequence. In RMSProp optimizer, $\eta$ is generally less likely to cause problems when $\eta > fp16_{min}$, but the denominator $v_t$,  adaptive learning rate, and $\epsilon$ can cause numerical instability when out of the available range. 
\begin{align*}
v_t =& {\begin{cases}
0 & if \: v_t < fp16_{min} \\
{\beta} {v_{t-1}} + {(1 - \beta) {{g_t}^{2}}} & otherwise\\
\infty & if \: v_t > fp16_{max}
\end{cases}}
\end{align*}
if ${v_t}$ is less than $fp16_min$, ${v_t}$ becomes $0$, and this effects $w_t$. The expression for $w_t$ is reorganized in such a way that only $\epsilon$ remains in the denominator. At this time, the numerical instability of this optimizer is caused by default $\epsilon$. In TensorFlow, the default value of $\epsilon$ is 1e-07, and the default learning rate $\eta$ is 1e-03. 
\begin{align*}
w_t =& w_{t-1} - \eta \cdot {g_t} \cdot {\epsilon}^{-1}
\end{align*} 
The weight is varied by the $\epsilon$ value. However, at this time, the numerical instability occurs when it becomes the reciprocal, which causes underflow and overflow in this optimizer. 
\begin{align*}
\epsilon^{-1} =& 
{\begin{cases}
\infty & if \: \epsilon^{-1} > fp16_{Max} \\
\epsilon^{-1} & otherwise \\
\end{cases}}
\end{align*}
If epsilon becomes 1e-07, the reciprocal of epsilon becomes 1e+07. In 16 bits, 1e-07 is acceptable, but 1e+07 generates an overflow and becomes $\infty$. An unconditional overflow occurs regardless of $g_t$, the gradient. This gradually creates numerical instability and breaks down the neural network. When $\epsilon^{-1} > fp16_{max}$, the $g_{t} \cdot \epsilon^{-1}$ should be $I = \{\infty, -\infty\}$ depending on the sign of $g_t$. 
\begin{align*}
w_t =& 
{\begin{cases}
w_{t-1} - \infty & if \: g_t > 0 \\
w_{t-1} + \infty & if \: g_t < 0 \\
\end{cases}}
\end{align*}
Current weight is $w_{t} = w_{t-1} - i$ ($i \in I$) and results in $\{NaN, -\infty\}$ when $w_{t-1} \in \{\infty, -\infty\}$. This optimizer will not work on the 16-bit neural network after $NaN$ occurs because the default epsilon of TensorFlow is set to 1e-07.

\textbf{Assumption 3.2} \textit{We assume that input image data $x \in X\{x_1,…,x_i\}$, label $y \in Y\{y_1,…,y_i\}$, all $x \in \mathbb{R}$, $0<x<255$, all $y \in \mathbb{Z}$. Data Normalized $\bar{x}$ will be range in $0.0<\Bar{x}<1.0$, and Gradient $g_t$ will be range in $fp16_{min}<g_t<fp16_{max}$. There are two situations for available 16-bit RMSProp. First of all, if $v_t \ne 0$, $v_t \ge fp16_{min}$ and $fp16_{min} < \sqrt{v_t} + \epsilon < fp16_{max}$, $w_t$ will not occur $overflow$. Secondly, when $v_t < fp16_{min}$, $v_t$ becomes $0$. If $g_t \cdot \epsilon^{-1} < fp16_{max}$, RMSProp avoids critical numerical instability. If either situation is satisfied, the RMSProp optimizer works on a 16-bit neural network.}

If \textbf{Assumption 3.2} is satisfied, RMSProp will work on 16-bit neural networks. The inappropriate epsilon can provide the wrong direction in overall 16-bit neural network learning. This results in a potential numerical instability and leads to the wrong conclusion that the RMSProp optimizer is not suitable for 16-bit neural network.

\subsubsection{Adam} 
Adam is an algorithm that combines RMSProp and Momentum methods. Adam is an alternative optimization algorithm that runs a repetitive cycle of adaptive moment estimation to provide more efficient neural network weights computation (Diederik, Kingma, \& Jimmy Ba). Adam extends to stochastic gradient descent to solve non-convex problems faster, using fewer resources than many other optimizers. This is most effective on large datasets by keeping the slope tighter on many training iterations.
\begin{align*}
w_t =& w_{t-1} - \eta \cdot \frac{\hat{m_t}}{\sqrt{\hat{v_t}} + \epsilon}
\end{align*} 
In the case of Adam, numeric instability occurs with a similar principle with RMSProp. The difference from RMSProp is that there is a Momentum variable $m$. In Adam, $m$ and $v$ are initially set to 0. Therefore, at the beginning of learning, $m_t$ and $v_t$ will be biased close to zero, and they first go through a process of making it unbiased. 
\begin{align*}
m_t =& \beta_1 \cdot m_{t-1}  + (1 - \beta_1) \cdot g_t \\ 
v_t =& {\beta_2} \cdot {m_{t-1}} + {(1 - \beta_2) \cdot {{g_t}^{2}}}
\end{align*}
Velocity $v_t$ is a non-negative real number. Because $\hat{v}_t$ is ${v_t}/{(1-\beta_{2})}$, if ${{v_t}}$ is less than $fp16_{max}$. ${\hat{v_t}}$ becomes $0$, and this effects $w_t$ value of the Adam optimizer.
\begin{align*}
w_t =& w_{t-1} - \eta \cdot \hat{m_t} \cdot {\epsilon^{-1}}
\end{align*}
If the $\epsilon^{-1} > fp16_{max}$, $\epsilon^{-1}$ is $\infty$. In TensorFlow, the default value of $\epsilon$ is $1e-07$, and the default learning rate $\eta$ is $1e-03$. $1e-07$ becomes $\infty$. According to the sign of $\hat{m_t}$, the momentum, $\eta \cdot \hat{m_t} \slash \epsilon$ becomes $\{\infty, -\infty\}$. The $\hat{m_t} \slash \epsilon$ should be $I = \{\infty, -\infty\}$  whatever the value of $\eta$. $w_{t} = w_{t-1} - i$ ($i \in I$) results in $\{NaN, -\infty\}$ when $w_{t-1} \in \{\infty, -\infty\}$. 
\begin{align*}
w_t =& 
{\begin{cases}
w_{t-1} - \infty & if \: \hat{m_t} > 0 \\
w_{t-1} + \infty & if \: \hat{m_t} < 0 \\
\end{cases}}
\end{align*}
This sequence results in a numerical instability in a 16-bit neural network. Thus, if $w_{t-1}$ is $-\infty$, $w_{t-1}$ - $\infty$ is $-\infty$, but $w_{t-1}$ + $\infty$ results in $NaN$. Thus, current $w_t$ is $NaN$. This Adam optimizer stop training on the 16-bit Neural Network.

\textbf{Assumption 3.3} \textit{We assume that input image data $x \in X\{x_1,…,x_i\}$, label $y \in Y\{y_1,…,y_i\}$, all $x \in \mathbb{R}$, $0<x<255$, all $y \in \mathbb{Z}$. $\bar{x}$ Normalized from $x$ will be range in $0.0<\Bar{x}<1.0$, and Moment $m_t$ will be range in $fp16_{min}<m_t<fp16_{max}$. There are two situations for available 16-bit Adam. First of all, if $\hat{v_t} \ne 0$, $\hat{v_t} \ge fp16_{min}$ and $fp16_{min} < \sqrt{\hat{v_t}} + \epsilon < fp16_{max}$, $w_t$ will not occur $overflow$. Secondly, when $\hat{v_t} < fp16_{min}$, $\hat{v_t}$ becomes $0$. If $\hat{m_t} \cdot \epsilon^{-1} < fp16_{max}$, Adam avoids critical numerical instability. If either situation is satisfied, the Adam optimizer works on a 16-bit neural network.}

Because Adam optimizer applied the RMSProp optimizer method, the 16-bit Neural Network does not work well for similar reasons. If Adam satify \textbf{Assumption 3.3}, the optimizer work on 16-bit Neural Network. If we understand the epsilon problem well as above, we can use various optimizers even in 16-bit computations. 


\subsection{REF TEMP}
Ruder, Sebastian. (2016). An overview of gradient descent optimization algorithms. 
Diederik P. Kingma and Jimmy Lei Ba. Adam: a Method for Stochastic Optimization. International Conference on Learning Representations, pages 1–13, 2015. \\
LeCun, Y., Bottou, L., Bengio, Y., $\&$ Haffner, P. (1998). Gradient-based learning applied to document recognition. Proceedings of the IEEE, 86(11), 2278-2324. \\
Krizhevsky, A., $\&$ Hinton, G. (2009). Learning multiple layers of features from tiny images. Technical report, University of Toronto.
Kingma, D. P., $\&$ Ba, J. (2014). Adam: A method for stochastic optimization. arXiv preprint arXiv:1412.6980.
Bottou, L. (2010). Large-scale machine learning with stochastic gradient descent. In Proceedings of COMPSTAT'2010 (pp. 177-186).
Chetlur, S., Woolley, C., Vandermersch, P., Cohen, J., Tran, T., Catanzaro, B., \& cuDNN Development Team (2014). cuDNN: Efficient Primitives for Deep Learning. arXiv preprint arXiv:1410.0759.

